Position Paper: Model Access should be a Key Concern in AI Governance

The downstream use cases, benefits, and risks of AI systems depend significantly on the access afforded to the system, and to whom. However, the downstream implications of different access styles are not well understood, making it difficult for decision-makers to govern model access responsibly. Consequently, we spotlight Model Access Governance, an emerging field focused on helping organisations and governments make responsible, evidence-based access decisions. We outline the motivation for developing this field by highlighting the risks of misgoverning model access, the limitations of existing research on the topic, and the opportunity for impact. We then make four sets of recommendations, aimed at helping AI evaluation organisations, frontier AI companies, governments and international bodies build consensus around empirically-driven access governance.

==> old.tex <==
The rapid development and adoption of general purpose artificial intelligence systems has prompted significant discussion about how to govern this technology \cite{AISummitNovember2023, USAIEO, EUAIAct}. A key concern has been to reduce the risk that AI systems create or facilitate societal harms, and ensure that they support diverse objectives \cite{anderljung2023frontierairegulationmanaging}.

When deployers release a model, they need to make decisions about which parts to make available, to whom \cite{shevlane2022structured}. For instance, one organisation might implement an access regime in which the public can only access a chat-style interface as part of larger system, whilst a second might share information about a model's weights and training data online. Different access styles might be provided to different stakeholders: for instance, internal company members, regulators, AI safety organizations, third-party researchers, and the public. We refer to these decisions about what to make available to whom as `model access governance'. 

Misgoverning model access could have serious consequences. On the one hand, releasing information about models incautiously could create more severe and difficult to manage risks \cite{seger2023opensourcinghighlycapablefoundation, kapoor2024societalimpactopenfoundation, davidevan}. On the other hand, over-cautious access regimes could create harmful opportunity costs \cite{fbOpenSource, mozillaJointStatement}. Experts have argued that both types of harms may become more likely over time, and could be difficult to reverse \cite{seger2023opensourcinghighlycapablefoundation, mozillaJointStatement}. As such, society may be at an inflection point, where setting out good governance principles early could have outsized benefits, whilst failing to do so could make it difficult to achieve societal goals. 

Despite this, decision makers are currently poorly positioned to navigate model access effectively. The small number of independent relevant research papers have been limited by a lack of empirical data, inadequate concepts, and limited breadth. As a result, decision makers are highly uncertain about the downstream implications of different styles of access, and have been slow to develop official guidelines for governing model access. For instance, although significant legislation acknowledges that model release should be proportional to risk \cite{rsp, USAIEO, EUAIAct}, there is no clear national law or industry commitment specifying how model deployers should apply this principle to the different access styles they choose to release.

The major obstacle to effective governance is uncertainty. There is significant uncertainty as to what styles of access are available, what use cases they might afford, and to whom. There is a further uncertainty as to how this might translate to real-world impacts, benefits, and costs for different groups. To remedy this situation, decision makers need more than lists of questions they don't know how to answer \cite{carnegieendowmentBeyondOpen}. Society needs a field of research set up to determine empirical inputs to address key uncertainties, and to build the processes necessary to support and ensure responsible decision making around model access as AI systems become more powerful over time.

Consequently, we introduce `Model Access Governance', a field of AI research helping organisations and governments to make responsible, evidence-based decisions about model access. Building on Alan Dafoe's definition of AI Governance \cite{dafoe2018ai}, Model Access Governance is a field of research looking to build policies, norms, laws, and institutions that shape who accesses which features of or what information about which AI models, when, and in what way, such that these decisions better achieve diverse societal objectives. We emphasize the importance of empirically driven, ethically conscious research with clear processes for organizations to implement.

In this paper, we make the case for researchers to work on Model Access Governance. We argue that the risks from misgoverning model access are severe and underestimated; that experts are currently uncertain about how to govern model access, as existing literature on the subject is limited; and that building a field of research could materially improve decision makers' abilities to govern model access effectively. Consequently, we recommend that i) deployers pre-evaluate access styles before release, ii) governments strengthen their ability to assess downstream use cases, and iii) international organizations build consensus on empirically-driven access governance. A final appendix gestures to six categories of open problems that researchers might prioritise. 


\begin{figure}
    \centering
    \includegraphics[width=01\linewidth]{image.png}
    \caption{Speculative results from an access-based model evaluation}
    \label{fig:enter-label}
\end{figure}

